Robustness-Runtime Tradeoff for Quantum State Transfer

Quantum state transfer is the primitive of transporting an unknown state on one site of a lattice to another. Using power-law interactions, recent state transfer protocols achieve speedup by utilizing the intermediate ancilla sites. However, these protocols require the ancillas to be in a perfectly initialized state, which, due to noise or imperfect control, may not be the case. In this work we introduce the $\textit{robustness}$ of a state transfer protocol, which quantifies the protocol's tolerance to error in the initial ancilla state. In the Heisenberg picture, state transfer grows operators supported on the final site such that they no longer commute with all operators on the starting site. We prove that this robustness tightly bounds the Schatten $p$-norms of these commutators between initial and final-site operators. This generalizes the known cases of $p=\infty$ and $p=2$, which govern completely state-dependent and state-independent state transfer respectively, demonstrating that intermediate values of $p$ govern partially state-dependent state transfer. In conjunction with existing power-law light cones, our result gives new minimum runtimes for partially state-dependent protocols which, in certain regimes, are parametrically better than existing bounds. We introduce new robust state transfer protocols, charting the landscape between complete state-dependence and state-independence.

==> preamble.tex <==
\usepackage{graphicx}
\usepackage[dvipsnames]{xcolor}
\usepackage{rotating}
\usepackage{amsmath,amssymb,graphics,amsthm}
\usepackage{amsfonts,dsfont,mathtools}
\usepackage{bbm}
\usepackage{bm}
\usepackage{array}
\usepackage{appendix}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\usepackage{multirow}
\usepackage{physics}
\usepackage{tikz-cd}
\usepackage{adjustbox}
\usepackage{stmaryrd}
\usepackage{tikz}
\usetikzlibrary{shadows.blur}



\usepackage[colorlinks=true, urlcolor=violet, linkcolor=blue, citecolor=red, hyperindex=true, linktocpage=true]{hyperref}
\usepackage[capitalise,compress]{cleveref}

\allowdisplaybreaks

\newtheorem{thm}{Theorem}
\numberwithin{thm}{section}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{hyp}[thm]{Hypothesis}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{eg}[thm]{Example}
\newtheorem{claim}[thm]{Claim}
\newtheorem{obs}[thm]{Observation}
\newtheorem{defn}[thm]{Definition}
\newcommand{\nn}{\nonumber\\}


\renewcommand{\thetable}{\arabic{table}}
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}
%\renewcommand{\theequation}{\thesection.\arabic{equation}}
\makeatletter
\renewcommand{\p@subsection}{}
\renewcommand{\p@subsubsection}{}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%% for this paper
\newcommand\ra{\rangle}
\newcommand\la{\langle}
\newcommand\bea{\begin{eqnarray}}
\newcommand\eea{\end{eqnarray}}
\newcommand\be{\begin{equation}}
\newcommand\ee{\end{equation}}
\newcommand\bes{\begin{subequations}}
\newcommand\ees{\end{subequations}}
\newcommand\bed{\begin{displaymath}}
\newcommand\eed{\end{displaymath}}
\newcommand\beal{\begin{aligned}}
\newcommand\eeal{\end{aligned}}
\newcommand\bew{\begin{widetext}}
\newcommand\eew{\end{widetext}}
\newcommand\beit{\begin{itemize}}
\newcommand\eeit{\end{itemize}}
\def\bea{\begin{array}}
\def\eea{\end{array}}
\newcommand\been{\begin{enumerate}}
\newcommand\eeen{\end{enumerate}}

\newcommand{\intxyt}{\int \mathrm{d}x \mathrm{d}y \mathrm{d}t}
\newcommand{\intxt}{\int \mathrm{d}x \mathrm{d}t}
\newcommand{\intxyzt}{\int \mathrm{d}x \mathrm{d}y \mathrm{d}z \mathrm{d}t }

\newcommand{\xt}{\tilde{X}}
\newcommand{\yt}{\tilde{Y}}
\newcommand{\stx}{\tilde{S}_x}
\newcommand{\He}{\rm{He}}

\newcommand{\eqnref}[1]{\eqref{#1}}
\newcommand{\figref}[1]{Figure\;\ref{#1}}
\newcommand{\tabref}[1]{Table\;\ref{#1}}
\newcommand{\secref}[1]{Section\;\ref{#1}}
\newcommand{\appref}[1]{Appendix\;\ref{#1}}

\newcommand{\ud}{\mathrm{d}}
\def\i{\text{i}}
%\newcommand\gaa{\gamma_{\text{e-ph}}}

% identity operator
\newcommand{\id}[0]{\mathds{1}}

\newcommand{\sr}{\text{sr}}
\newcommand{\lr}{\text{lr}}
\newcommand{\CNOT}{\textsc{CNOT}}
\newcommand{\vac}{\text{vac}}
\newcommand{\cj}{\text{c.j.}}
\newcommand{\ii}{\mathrm{i}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\bracket}[1]{\left(#1\right)}

\usepackage{verbatim}

\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\im}{\mathrm{Im}~}
\newcommand{\re}{\mathrm{Re}~}
%\newcommand{\dd}{\delta}
\newcommand{\eps}{\epsilon}
\newcommand{\para}{\parallel}
\newcommand{\phan}{\phantom{i}}

\newcommand{\p}{\partial}

% Transpose
\newcommand{\transpose}[0]{\mathsf{T}}

\usepackage{tikz}
\usetikzlibrary{quantikz2}

% Green check mark
\definecolor{red1}{rgb}{0.76, 0.23, 0.13}
\definecolor{green1}{rgb}{0.0, 0.5, 0.0}
\usepackage{pifont} % http://ctan.org/pkg/pifont
\newcommand{\cmark}{\textcolor{green1}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red1}{\ding{55}}}

% Tables
\usepackage{booktabs}
